Convolutional Bayesian Kernel Inference for 3D Semantic Mapping

Robotic perception is currently at a cross-roads between modern methods, which operate in an efficient latent space, and classical methods, which are mathematically founded and provide interpretable, trustworthy results. In this paper, we introduce a Convolutional Bayesian Kernel Inference (ConvBKI) layer which learns to perform explicit Bayesian inference within a depthwise separable convolution layer to maximize efficency while maintaining reliability simultaneously. We apply our layer to the task of real-time 3D semantic mapping, where we learn semantic-geometric probability distributions for LiDAR sensor information and incorporate semantic predictions into a global map. We evaluate our network against state-of-the-art semantic mapping algorithms on the KITTI data set, demonstrating improved latency with comparable semantic label inference results.

==> Background.tex <==
\section{Literature}
In this section, we provide background knowledge on Bayesian Kernel Inference (BKI) and neural network loss functions. 

\subsection{BKI} \label{sec:BKI_Literature}
Maps traditionally use a binary occupancy representation, however some works consider embedding semantic segmentation information. One method is to use Gaussian Process (GP) Occupancy Mapping \cite{GaussianProcessOccupancyMaps}, which fits Gaussian functions to the training data ${x_i, y_i}$ where $x_i$ is the position and $y_i$ is the label of a point. This is computationally intensive however, resulting in cubic $O(n^3)$ complexity with the number of data points. A faster alternative is to approximate GP's using Bayesian Kernel Inference (BKI) in $O(logN)$ computations \cite{BKI}. This method has been applied to mapping in BGKOctoMap \cite{BGKOctoMap} and SemanticBKI \cite{SemanticBKI}. 

In SemanticBKI, the world is divided into discrete 3D cells (voxels), where each voxel has a categorical distribution for semantic segmentation. A Dirichlet distribution is maintained for the voxel as it is the conjugate prior of the categorical distribution, and yields a Dirichlet posterior in Bayesian inference. Additionally, the Dirichlet distribution has closed-form mean, mode (MAP), variance, and entropy. Instead of approximating the model during inference, the approximation is made during model selection. 

The baseline method is the Semantic Counting Sensor Model (S-CSM), which increments $\alpha$ parameters of the Dirichlet distribution by counting observations within the cell. The drawback is that data is only used to update the cell it falls in, and cells are assumed independent from each-other. BKI imposes a smoothness constraint relating the extended likelihood $p(y_i | \theta_*, x_i, x_*)$ and likelihood $p(y_i | \theta_i)$. After some math, the end result is that:

\begin{equation}\label{eq:BKI update}
    \alpha_*^k := \alpha_0^k + \sum_{i=1}^{N} k(x_*, x_i) y_i^k
\end{equation}

where $k$ is the kernel function, $i$ is the i-th data point, $y$ is the semantic label, $*$ is the query voxel. The kernel doesn't need to be \emph{positive definite or symmetric} \cite{KernelDerivation}, and is chosen in SemanticBKI to be the sparse kernel \cite{SparseKernel}. The only requirements are that:

\begin{equation}\label{eq:Requirement 1}
    k(x, x) = 1 \forall{x}
\end{equation}

\begin{equation}\label{eq:Requirement 2}
    k(x, x') \in [0, 1] \forall x, x'
\end{equation}

The authors argue the proposed method can handle sparse and noisy measurements, and query at arbitrary resolution. This method works well in a static environment, but can't handle dynamic objects. 

\subsection{Radius Neighborhoods}
BKI relies on the ability to query points in a ball about each voxel in real time, and compute a kernel over the neighboring points in real time. Several deep learning architectures have already incorporated a radius neighborhood search in feature or Euclidean space, including PointNet++ \cite{PointNet++}, DGCNN \cite{EdgeConv}, and KPConv \cite{KPConv}. 

Kernel Point Convolution (KPConv) \cite{KPConv} is a network architecture which implements convolution directly on point clouds without an intermediate representation such as voxels. Convolution is applied in continuous space over a ball about the query point $x$. The convolution operator is defined as follows:

\begin{equation}\label{eq:KPConv}
    (\mathcal{F} * g) (x) = \sum_{x_i \in \mathcal{N}_x} g(x_i - x) f_i
\end{equation}

\begin{equation}\label{eq:ConvNeighborhood}
    \mathcal{N}_x = \{ x_i \in \mathcal{P} \,\mid\, ||x_i - x|| \leq r \}
\end{equation}

$\mathcal{N}_x$ is a set containing all points $x_i$ in the point cloud $\mathcal{P}$ within a radius neighborhood $r$ about query point $x$. The convolution operator computes a weighted sum of the feature vectors associated with each local point. The weighted transformation is computed by kernel function $g$. Kernel function $g$ is defined as follows, where $y_i = x - x_i$:

\begin{equation}\label{eq:KPKernel}
    g(y_i) = \sum_{k < K} h(y_i, \tilde{x_k}) W_k
\end{equation}

\begin{equation}\label{eq:Anchors}
   h(y_i, \tilde{x_k}) = \text{max} \left( 0, 1 - \frac{||y_i - \tilde{x_k}||}{\sigma} \right)
\end{equation}

$W_k$ is a weight matrix to transform the feature vector dimensionality of $f_i$ from $D_{in}$ to $D_{out}$. The kernel function computes local weights from anchor points $\tilde{x_k}$. 

PointNet++ applies a similar radius neighborhood operation. Given a point cloud with a feature vector for each point, it outputs a new set of feature for each point in the input point cloud. For each point, neigbors within a ball are grouped, and a PointNet \cite{PointNet} operation is applied to produce a new feature vector. 

DGCNN incorporates an EdgeConv layer which computes a k Nearest Neighbor (kNN) search entirely in feature space. While a radius neighborhood or ball search applies the same spatial function to each point, a kNN search may incorporate further points or discard neighbors. 

To operate on large point clouds, all of the above operations must be highly efficient. In practice, the methods use either small point clouds or downsampling, as the computation cost explodes with the number of input and query points. DGCNN doesn't downsample, but uses point clouds of size 1,024 points. KPConv performs operations on an average point cloud size of 6,800 points with grid subsampling. PointNet++ downsamples points with iterative furthest point subsampling (FPS).   

\subsection{Explicit and Implicit Representations}
Maps can be constructed using explicit or implicit geometric representations. Explicit representations discretize the map into cells which may be directly queried. Implicit representations use a latent state which may be queried with continuous coordinates. While explicit representations are generally used by hand-crafted methods, implicit representations are typically part of deep learning mapping algorithms. 

Explicit representations provide human-interpretable states at the cost of memory and computation. Representing a map in higher dimensional space comes with an exponential cost as the dimensionality grows. Thus, maps are usually constrained to coarse representations. They also provide benefits, such as the ability to compute Bayesian inference as in Semantic BKI \cite{SemanticBKI} or K3DOM \cite{K3DOM}. These maps are able to quantify uncertainty at every step, and increase trustworthiness due to their repeatability and interpretability. While explicit maps may not maximize memory efficiency, they are not likely to break given spurious data. 

Implicit representations on the other hand, are generative models which implicitly encode the geometry of a scene. They may be queried in continuous space, and are increasingly popular in deep learning architectures. Some examples include Neural Radiance Fields (NeRF) \cite{NERF, BlockNERF} and implicit occupancy mapping algorithms \cite{VoxBlox, NeuralBlox, ImplicitOccupancyCNN}.  NeuralBlox is a recent deep learning mapping algorithm which uses implicit representations to update an occupancy map in real time. NeuralBlox encodes 3D input data to a latent space, which is fused temporally to calculate hidden states of an occupancy grid. The hidden states may then be queried in continuous space to generate occupancy points. 

While implicit representations can train a real-time occupancy mapping algorithm, they comes with some drawbacks. Firstly, although implicit representations are supposedly more memory efficient, the hidden states of occupancy maps are still stored in a discrete grid \cite{NeuralBlox}. The memory improvement then depends on the size of the hidden state of each voxel, and there is a trade-off between resolution and feature vector size. Next, explicit Bayesian inference cannot be computed on the hidden state, resulting in an occupancy probability without a quantifiable uncertainty. Finally, these mapping methods do not directly leverage advances in lower level scene understanding tasks such as semantic segmentation or object detection. 

\subsection{Losses}

Because the kernel is typically hand tuned on data, we believe that the kernel naturally lends itself to be optimized through learning based methods. This leads to our motivation for defining a suitable loss function. Many works \cite{UNet2015, } have successfully used cross entropy to train pixel level classification and segmentation. While effective at measuring the difference between two probability distributions, cross entropy loss tends to spread out its probability distribution to avoid a high loss, whereas we desire a loss function that directly minimizes variance for each cell. Another interesting loss is Correlated Maximized Structural Similarity loss. This method \cite{ZhaoShuai2019} attempts to incorporate structural information at a pixel level to weight the cross entropy loss function. Therefore, minimizing the loss still does not directly relate to minimizing the variance. Many likelihood based frameworks like \cite{9244048, Razali_2021_WACV} have used a log likelihood version KL divergence as a loss term. We assume that the prior and posterior for each cell should follow the same distribution, so enforcing this loss would maximize the likelihood of our prior estimate given new measurements. Applying this loss term offers a nice intuition that if the kernel's prediction is representative of the underlying map distribution, then subsequent measurements of the map should provide little information gain, thus leading to a lower loss.   

\begin{equation}\label{entropy:1}
    H(X) = log(B(\alpha)) + (\alpha_0 - K) \phi(\alpha_0) - \sum_{j=1}^K (\alpha_j - 1) \phi(\alpha_j)
\end{equation}

Because minimizing variance is equivalent to maximizing entropy defined in equation \ref{entropy:1}, it is beneficial to use the inverse of entropy as a term in our loss function. Because we assume a Dirichlet prior and posterior distribution for P and Q, we know the closed form solution for the posterior cross entropy for each map cell i. This makes computing the loss for each cell highly efficient

